Combining Sampling- and Gradient-based Planning for Contact-rich Manipulation

Planning over discontinuous dynamics is needed for robotics tasks like contact-rich manipulation, which presents challenges in the numerical stability and speed of planning methods when either neural network or analytical models are used. On the one hand, sampling-based planners require higher sample complexity in high-dimensional problems and cannot describe safety constraints such as force limits. On the other hand, gradient-based solvers can suffer from local optima and convergence issues when the Hessian is poorly conditioned. We propose a planning method with both sampling- and gradient-based elements, using the Cross-entropy Method to initialize a gradient-based solver, providing better search over local minima and the ability to handle explicit constraints. We show the approach allows smooth, stable contact-rich planning for an impedance-controlled robot making contact with a stiff environment, benchmarking against gradient-only MPC and CEM.

==> archive.tex <==
\section{Introduction}\label{Introduction}
Many manipulation tasks require physical interaction between the manipulator and the environment. Tasks such as door opening, surface finishing operations, insertion of tight-fitting parts, and mating of gears require significant interaction with the environment and involve complex dynamics. However, traditional manipulation framework is developed considering minimal interaction with the environment. This limits the application of manipulator arms to a constrained and well-defined environment with precise kinematic motions. In contrast, human manipulation has no such limitations and efficiently engage in a task that involves physical interaction with the environment. This serves as the motivation for developing manipulation methods that actively interact with the environment by explicitly considering interaction phenomena such as stiffness, surface contacts, and impacts. This physical interaction is complex, with contact being made and broken during a trajectory, and where the contact parameters may be uncertain. The highly non-linear nature of such interaction dynamics results in large discontinuities in the dynamics during contact transitions, in the form of high forces, jerk and vibrations.

These sudden and uncontrolled system disturbances during contact change instances such as collisions can damage the robot and/or objects involved.
An ideal planning framework for executing a contact-rich task should therefore be able to follow the provided plan while ensuring that: (i) it can handle the discretely changing interaction dynamics that arise when the robot is engaging and breaking contact with an object/environment; (ii) it can safely plan actions while ensuring multiple levels safety constraints.

\subsection{Related works}
Model-based planning for contact-rich robotic tasks consists of finding the action sequence that minimizes a cumulative cost function, according to learned or parametrized dynamics. Usually, optimized actions are executed with model predictive control (MPC), replanning at each time step. However, these planning problems are usually to complex to solve optimally due to highly nonlinear/discontinuous dynamics, continuous action spaces and possibly non-convex cost functions. In case of demanding tasks, this problem could be completely unacceptable, as sub-optimal solutions could potentially lead to high contact forces with subsequent task failure. 

For these tasks, a possible solution for finding the optimal action sequences is the family of population-based sampling methods such as Random-Sampling Shooting Method (RS) (Nagabandi et al., 2018), Model Predictive Path Integral Control (MPPI) (Williams et al., 2017), and Cross-Entropy Method (CEM) (Rubinstein, 1997).

Fundamentally, these zeroth-order optimizers are variants of CEM, which maintains a sampling distribution to sample rollouts of action sequences (Okada and Taniguchi, 2020). This sampling distribution is updated at each iteration to assign a higher probability near higher reward action sequences. In recent years, there has been a huge research effort on sampling based optimization in the context of model-based reinforcement learning. The work of (cite iCEM paper) have developed an improved version of the CEM algorithm for fast planning with novel additions including temporally correlated actions and memory. Results show that the proposed algorithm requires approximately 2.7-22X less samples and yields a performance increase of 1.2-10X in high dimensional control
problems. In (cite Loris paper w CEM), authors proposed a model-based reinforcement learning approach in which the interaction dynamics was directly learned through an ensemble of Artificial Neural Networks (ANNs). In order to exploit the learned model within an online planning framework a Cross Entropy Method (CEM) was used to optimize the impedance parameters with respect to human effort. 

However, CEM, like all sampling-based planners, suffers from scalability for high-dimensional problems (Bharadhwaj et al., 2020). As the dimension of the action space and/or the planning horizon grows, many more samples are needed for CEM-based planners to converge, and the variance in the reward of CEM-based planners increases (Bharadhwaj et al., 2020; Chua et al., 2018). This effect makes it difficult to use CEM with long planning horizons if the number of samples taken by CEM is fixed (Chua et al., 2018). Scalability is a fundamental drawback of zeroth-order optimizers, and poses a significant challenge to real-time planning when computation time is a constraint, e.g., when parallelization is not possible. 

Gradient-based methods are often used effectively on high-dimensional optimization problems, in presence of a differentiable dynamics model and cost function and have also been applied to contact-rich planning. Authors in (cite Kevin paper on gp-mpc) effectively used a first order MPC framework for planning actions with respect to human goal belief. The proposed planning framework allows to enforce multiple levels of safety constraints, as first order methods easily handle state and input dependent constraints if compared with sampling-based solvers. However, the main problem when trying to optimize very complex and nonlinear learned models is that they strongly dependent on the data acquired for the training phase, making the generalization to new trajectories or adaptation to variation in geometric parameters uncertain. Gradient-based solvers can also get stuck in local minima, which could potentially be dangerous for certain tasks.

For planning in contact, recent work \cite{suh2022a} has shown that first order methods can have higher variance than zeroth order methods at higher stiffness and in longer planning horizons. 

An interesting idea is to combine zeroth-order and first-order planning methods in order to enjoy the benefits of both simultaneously. To this end, authors in (Bharadhwaj et al. (2020) and cem+grad paper) proposed a combined planning framework that performs gradient updates on the sampled trajectories. Although able to exploit the advantages of both approaches, these methods still show scalability issues with very high dimensional planning problems.

\subsection{Paper contribution}
In this paper, we propose an innovative scalable hybrid planner that uses an improved version of the CEM-algorithm (cite iCEM paper) for the warm start of a nonlinear optimization problem solved with MPC. The manipulation task is modelled with a hybrid dynamics model framework, with discrete interaction dynamics according to different contact conditions. The MPC planner optimizes actions by minimizing the expectation over multiple cost transcriptions according to a belief about the contact mode. Within this framework, at each time step $t$ a CEM step is performed by first sampling and then rolling out $n$ action sequences according to different interaction dynamics, thus increasing the variability of the optimization landscape. The best action sequence along with its corresponding state trajectory are then used to warm start the MPC problem, with the aim of improving the convergence behaviour at contact transitions while at the same time achieving safer behaviours. The optimal action sequence found by the MPC planner is then used to update the mean of the CEM sampling distribution, thus increasing the likelihood of sampling optimal sequences.

